Domain-specific Communication Optimization for Distributed DNN Training

Communication overhead poses an important obstacle to distributed DNN training and draws increasing attention in recent years. Despite continuous efforts, prior solutions such as gradient compression/reduction, compute/communication overlapping and layer-wise flow scheduling, etc., are still coarse-grained and insufficient for an efficient distributed training especially when the network is under pressure. We present DLCP, a novel solution exploiting the domain-specific properties of deep learning to optimize communication overhead of DNN training in a fine-grained manner. At its heart, DLCP comprises of several key innovations beyond prior work: e.g., it exploits {\em bounded loss tolerance} of SGD-based training to improve tail communication latency which cannot be avoided purely through gradient compression. It then performs fine-grained packet-level prioritization and dropping, as opposed to flow-level scheduling, based on layers and magnitudes of gradients to further speedup model convergence without affecting accuracy. In addition, it leverages inter-packet order-independency to perform per-packet load balancing without causing classical re-ordering issues. DLCP works with both Parameter Server and collective communication routines. We have implemented DLCP with commodity switches, integrated it with various training frameworks including TensorFlow, MXNet and PyTorch, and deployed it in our small-scale testbed with 10 Nvidia V100 GPUs. Our testbed experiments and large-scale simulations show that DLCP delivers up to $84.3\%$ additional training acceleration over the best existing solutions.

==> sections/discussion.tex <==
\section{Discussion and Future Work}
\label{sec:design}

\textbf{Scheduling among different jobs.}

\textbf{Model parallel.}

\textbf{\sys for other general distributed tasks.}




==> sections/introduction.tex <==
\section{Introduction}

Modern machine learning trains complex models (\eg deep
neural networks) by iteratively applying stochastic 
gradient descent (SGD) to refine the model parameters~\cite{SGDopt}.
This process, however, is known to be frustratingly 
slow:
despite being easily parallelizable, the training 
algorithms must synchronize massive amounts of 
parameter updates across distributed workers (10s to 
100s) at the end of each iteration, creating potential 
congestion and in the worst case, 1-2 orders of 
magnitudes of slowdowns on the entire training process.

% Many popular ML models are trained using distributed {\em stochastic gradient descent (SGD)} at a large scale~\cite{tensorflow,mxnet,petuum}, but such SGD-based model training can be frustratingly slow.
% One reason is that large-scale distributed SGD requires intensive communication at the end of every iteration to synchronize and update huge amounts of parameters among the workers. 
% Thus, reducing the cost of the network communication is crucial to the performance of ML training.

Therefore, trimming the communication overhead for ML
training has gained much attention, in both ML and 
systems communities. 
Many ML-inspired solutions exploit the property that SGD-based training produces equally accurate models, 
even in the presence of a non-trivial amount of 
delayed, missed or lower-precision updates~\cite{qsgd2017nips,terngrad2017nips,sparse2018nips,deep2017arxiv}.
In the meantime, systems community has explored 
alternative communication patterns to mitigate traffic
hotspots~\cite{ps2014osdi,ring2018arxiv,petuum}. 
While being effective, neither approach addresses the 
real culprit: 
{\em tail flow completion time}, which are caused by 
transient traffic bursts (due to self-inflicted or 
competing applications) and plague modern high-speed
datacenters~\cite{dctcp,detail2012sigcomm}.
Thus, compressing parameter updates or optimizing parameter communication patterns is necessarily incomplete.

% The need to speedup network communications for distributed machine learning applications has inspired enormous efforts on the application level \cite{qsgd2017nips,terngrad2017nips,sparse2018nips,deep2017arxiv} and scheduling strategy \cite{ps2014osdi,ring2018arxiv}. 
% However, the gain of these efforts are limited by the performance of {\em transport layer protocols}. 
% In data center networks, reducing the amount of data may result in similar communication time due to retransmissions induced by incasts and sporadic packet drops. 

\parab{Why a transport-layer solution?}
In this paper, we argue that a {\em transport-layer}
solution is fundamentally needed to trim
the communication overhead in ML training. 
The key insight is that we can completely avoid tail
flow completion time, if the transport layer simply
ignores the fraction of data delayed or missed by the 
network.
First, doing so will not affect the training outcome 
(\ie same final accuracy and same number of 
iterations), as long as the amount of ignored data does
not exceed some threshold (typically, $10\%-35\%$).
Second, default transport protocols only offer 
``all-or-nothing'' semantics, leaving any solutions 
above transport layer unable to circumvent the tail 
latency. 
Note that these arguments do not apply to general data 
analytic applications (\eg MapReduce) in which data
communication must be reliable. 


% In this paper, we argue that {\em the transport-layer protocols should be deeply integrated with the need of large-scale distributed SGD}. 
% The key insight is that distributed SGD can tolerate a {\em bounded amount} of information loss when updating the parameters. We found that across a wide range of SGD-trained models, if the updates of $10\%-35\%$ parameters are lost in each iteration, the application performance is not affected.
% % This feature was insofar exploited only at the application level, and transport protocols can significantly reduce the flow completion time by embracing such bounded loss-tolerance feature. 

\parab{Why a new transport-layer design?}
These desirable behaviors, however, do not match 
existing transport-layer techniques.
The mismatch stems from the {\em bounded loss 
tolerance} property exhibited by SGD-based training---the 
utility of a flow is determined by the time needed
to transfer a predefined fraction $p<100\%$ of all
data, not by the time to transfer all data.
In contrast, TCP and its variants seek to minimize the
time to transfer all data ($p=100\%$), which 
inevitably suffers from tail latency even under a 
tiny fraction of packet delays/losses.
UDP, on the other hand, does tolerate tail effect, 
but without the guarantee that at least $p$ data must
be delivered, which can result in poor eventual 
accuracy and/or require more iterations to converge.


% The bounded-loss tolerance of SGD has several significant implications for congestion control protocols. 
% First, it opens up new avenues to dramatically improving the congestion control performance.
% Traditionally, Reliable Data Transfer (RDT) protocols, e.g. TCP, are susceptible to even a tiny amount of packet losses or latency inflation, which can stall a flow with just a few retransmissions. 
% In contrast, SGD's inherent loss tolerance allows transport protocols to safely ignore packet losses or delays up to a certain amount ($10\%$ to $35\%$), which exceeds the packet loss rate seen in today's data centers. 
% This could dramatically cut the tail flow completion time.

% At the same time, we argue that imbuing the bounded loss tolerance in transport protocols calls for expanding the congestion control with a correspondingly new semantic.
% Instead of minimizing the flow completion time, a bounded-loss tolerant congestion control minimizes the time by which the receiver get a given fraction $p$ of all packets. 
% \footnote{Similar notion has been explored in early research on video streaming, sensor data aggregation, and redundant packet coding~\cite{rpt2012nsdi,sensor2002icdcs}, but as we will see, they are not directly applicable in high-speed data centers or for ML training. }
% This essentially points to a new utility function of a network flow---the utility of a network flow is determined by the time upon receiving a predefined fraction of data. 
% To our best knowledge, this is the first definition on bounded loss tolerance of transport protocol in data center settings.

In the rest of this short paper, we start with understanding the initial promise of a better transport-layer approach. Using large scale NS-3 simulations, we show a bounded-loss tolerance transport protocol can produce 1.1-2.2x speedup on different ML tasks under simplified assumptions. The simplified protocol significantly reduces the tail latency by tolerating bounded packet losses. 
With an analysis on the message contents of distributed ML jobs, we show a bounded-loss protocol can provide valid information for ML applications in presence of discrete packet drops. 
We then discuss related works and call upon this community to develop transport layer solutions for distributed ML leveraging such bounded-loss tolerance feature. 

% Stochastic Gradient Descent (SGD)-based optimization algorithms \cite{SGDopt,Adamopt,Momentumopt,Nesterovopt} are widely used in training models in machine learning~\cite{tensorflow,mxnet,petuum}. 
% but such SGD-based model training can be frustratingly slow, especially when many workers coordinate to train the same model.
% One reason is that large-scale distributed SGD requires intensive communication at the end of every iteration to synchronize and update huge amounts of parameters among the workers and a master server. 

==> sections/junchen/design_jc.tex <==
\begin{figure*}[t]
\subfloat[Speedup under PS scheme]{
	\includegraphics[width=0.32\textwidth]{figures/PS_FCT.pdf}
	\label{subfig:mlt_ps}
}
\subfloat[Speedup under RING scheme]{
	\includegraphics[width=0.32\textwidth]{figures/RING_FCT.pdf}
	\label{subfig:mlt_ring}
}
\subfloat[FCT of simplified protocol and TCP (model:MLP)]{
    \includegraphics[width=0.32\textwidth]{figures/FCT2.pdf}
	\label{subfig:mlt_fct}
}
\caption{Speedup of simplified protocol against TCP}
\label{fig:mlt}
\end{figure*}
\section{Towards bounded-loss tolerant protocol}
\label{sec:design}

In this section, we discuss the potential of a bounded-loss tolerant protocol. The bounded-loss tolerant protocol should guarantee the delivery of a predefined fraction of data while delivering the rest of the data in a best effort manner. The protocol should handle packet losses as follows:

\begin{itemize}
    \item Packet losses that can be quickly detected (e.g., duplicated ACKs) will be retransmitted as original.
    \item {\em Bounded} packet losses with long detection time (e.g., retransmission timer) can be directly discarded. 
\end{itemize}
In this section, we demonstrate the advantages of an simplified protocol over existing protocols. We then discuss some challenges of integrating a bounded-loss tolerant protocols with ML application, and the intuition why it is tractable.

\subsection{Potential improvements}
\label{subsec:improvement}
Bounded-loss tolerance feature opens new avenues to congestion control design. Below a certain loss rate, unrecovered packet drops will not affect ML application performance. Since message size is purely determined by the ML model, in theory receivers are capable of deciding when the received data is enough to guarantee application level performance. 

We quantify the full potential of a bounded-loss tolerant protocol using an {\em simplified} version. The simplified protocol has no packet ordering requirements and only counts received data amount. 
The simplified protocol sends all data at sender side, enables fast retransmission mechanisms, and we measure the time when a predefined fraction $p$ of total data is received. The tolerance bound $p$ follows table~\ref{table:diffmodel}. 

\parab{Experimental settings. } We simulated an oversubscribed spine-leaf topology with 4 spine switches, 8 leaf switches and 16 servers in each rack. Within the same rack 8 servers generate distributed machine learning traffic, the other servers 
generate background traffic for other applications. 
These applications create a load factor of 0.5 on core links.
The over subscription ratio is 4:1. All the links in the topology is 40Gbps link. 
The switch buffer is configured of size 450KB, with an ECN marking threshold of 90KB. Default protocol is DCTCP with initial window of 10 packets.
We generate realistic workloads of data center same as \cite{dctcp} and employ Equal Cost Multi Path (ECMP) for load balancing.

The detailed hyper parameter settings can be found in table~\ref{table:model-detail}. We use fixed learning rate without weight decay and momentum factors. The convergence of ML jobs are defined to be the validation loss (i.e. model loss on a subset of data not used for training) decreases to a model-specific threshold. 
Each model is trained for 100 epochs. 

\parab{Estimating job completion time.} We run the ML jobs simulating packet drops as~\S\ref{subsec:loss} until the loss value is smaller than baseline (ML jobs without data losses) and epochs passed is no smaller than baseline.
The simulated job completion time is then
\begin{equation}
    \textrm{\# epochs} \times \big( \textrm{Compute time} + 2 \times \textrm{Network time} \big)
\end{equation}
We run a simulated ML jobs offline with real data, while emulating the data drops for each parameter uniformly at random. The random data loss rate is set as tolerance bound in table~\ref{table:diffmodel}.

\begin{table}[t]
\centering
\small
\begin{tabular}{|l|l|l|l|}
\hline
Abbrv. & Dataset & Batch Size & Learning Rate \\ \hline
MF & ~\cite{movielens} & 256 & 0.1 \\ \hline
MLP & ~\cite{reuters} & 32 & 0.5 \\ \hline
CNN & ~\cite{cifar10} & 32 & 0.1 \\ \hline
RNN & ~\cite{englishfrench} & 32 & 0.25 \\ \hline
\end{tabular}
\caption{Detailed models for evaluation}
\label{table:model-detail}
\end{table}

\parab{Preliminary results. } Figure~\ref{fig:mlt} shows the improvements against TCP when we run the models in table~\ref{table:model}. We compare the performance of the simplified protocol with the performance of TCP.
We find that leveraging the loss tolerant feature of SGD can greatly benefit distributed ML jobs.
For the models we select, the simplified protocol brings $1.1$x-$2.2$x speedups. 
The results of different parameter schemes are very similar. 
Due to the difference in the time spent in computation and communication in each model, we see different speedups for different models. 
Figure~\ref{subfig:tcp_udp} shows that the simplified protocol gets faster speed than TCP and provides a better application level performance than UDP. 

In figure~(\ref{subfig:mlt_fct}), we plot compare the flow completion time of all the flows generated by the MLP jobs. 
As figure shows, the main benefit of the simplified protocol is to cut the tail latency. The average FCT is similar with that of TCP. 
Therefore, the simplified protocol is effective in cutting the tail completion time of ML message transfers.

\subsection{Challenges}
Implementing a loss tolerant protocol is faced with an important challenge. As the protocol only specifies the highest loss rate tolerated, the received packet contents may contain multiple fragments that of the original message. In other words, the server may have received enough message in terms of size, but how to interpret the message remains a problem. 

Is it possible to understand the partially received message? The answer is positive. 
The key observation is that machine learning messages can be abstracted as a vector describing the model. The vector contains floating point numbers of 32 bits or smaller size. To interpret packets' content independently, it is sufficient to restrict that the same floating point number is not segmented into two packets. For example, a packet with $1400$ bytes of payload size is capable to contain 350 32-bit floating point numbers. In such cases, switching a on-the-boundary value to next packet reduces the packet size by less than $0.5\%$, meaning the additional packets generated by this requirement is negligible. 

\parab{Idea \#1: Range indexing of packets.} 
Following the vector abstraction of ML models, 
each packet contains two integer values as ranged keys indicating the index range of the packet's content in the vector. 
%Figure~\ref{fig:MLT-packet} illustrates this format. 
The overhead of inserting ranged key index is low: 
With a normal packet payload size of $\sim 1400$ bytes, adding two 32-bit numbers as ranged index increases the overhead of less than $1\%$, an negligible overhead to network traffic.

\parab{Idea \#2: Integrating with ML frameworks.} Upon receiving enough packets, the bounded loss tolerant should forward the received message to upper layer application, i.e., the ML frameworks. In addition, the transport protocol marks the index ranges that the data is not received. This gives the ML application the information required to take average of received gradients on server side, or to use an earlier version of parameter value on worker side.  

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figures/MLT_packet.pdf}
    \caption{A ranged indexing scheme for packets.}
    \label{fig:MLT-packet}
    \vspace{-5mm}
\end{figure}


==> sections/junchen/intro_junchen.tex <==
\section{Introduction}

Modern machine learning trains complex models (\eg deep
neural networks) by iteratively applying stochastic 
gradient descent (SGD) to refine the model parameters~\cite{SGDopt}.
This process, however, is known to be frustratingly 
slow:
despite being easily parallelizable, the training 
algorithms must synchronize massive amounts of 
parameter updates across distributed workers (10s to 
100s) at the end of each iteration, creating potential 
congestion and in the worst case, 1-2 orders of 
magnitudes of slowdowns on the entire training process.

% Many popular ML models are trained using distributed {\em stochastic gradient descent (SGD)} at a large scale~\cite{tensorflow,mxnet,petuum}, but such SGD-based model training can be frustratingly slow.
% One reason is that large-scale distributed SGD requires intensive communication at the end of every iteration to synchronize and update huge amounts of parameters among the workers. 
% Thus, reducing the cost of the network communication is crucial to the performance of ML training.

Therefore, trimming the communication overhead for ML
training has gained much attention, in both ML and 
systems communities. 
Many ML-inspired solutions exploit the property that SGD-based training produces equally accurate models, 
even in the presence of a non-trivial amount of 
delayed, missed or lower-precision updates~\cite{qsgd2017nips,terngrad2017nips,sparse2018nips,deep2017arxiv}.
In the meantime, systems community has explored 
alternative communication patterns to mitigate traffic
hotspots~\cite{ps2014osdi,ring2018arxiv,petuum}. 
While being effective, neither approach addresses the 
real culprit: 
{\em tail flow completion time}, which are caused by 
transient traffic bursts (due to self-inflicted or 
competing applications) and plague modern high-speed
datacenters~\cite{dctcp,detail2012sigcomm}.
Thus, compressing parameter updates or optimizing parameter communication patterns is necessarily incomplete.

% The need to speedup network communications for distributed machine learning applications has inspired enormous efforts on the application level \cite{qsgd2017nips,terngrad2017nips,sparse2018nips,deep2017arxiv} and scheduling strategy \cite{ps2014osdi,ring2018arxiv}. 
% However, the gain of these efforts are limited by the performance of {\em transport layer protocols}. 
% In data center networks, reducing the amount of data may result in similar communication time due to retransmissions induced by incasts and sporadic packet drops. 

\parab{Why a transport-layer solution?}
In this paper, we argue that a {\em transport-layer}
solution is fundamentally needed to trim
the communication overhead in ML training. 
The key insight is that we can completely avoid tail
flow completion time, if the transport layer simply
ignores the fraction of data delayed or missed by the 
network.
First, doing so will not affect the training outcome 
(\ie same final accuracy and same number of 
iterations), as long as the amount of ignored data does
not exceed some threshold (typically, $10\%-35\%$).
Second, default transport protocols only offer 
``all-or-nothing'' semantics, leaving any solutions 
above transport layer unable to circumvent the tail 
latency. 
Note that these arguments do not apply to general data 
analytic applications (\eg MapReduce) in which data
communication must be reliable. 


% In this paper, we argue that {\em the transport-layer protocols should be deeply integrated with the need of large-scale distributed SGD}. 
% The key insight is that distributed SGD can tolerate a {\em bounded amount} of information loss when updating the parameters. We found that across a wide range of SGD-trained models, if the updates of $10\%-35\%$ parameters are lost in each iteration, the application performance is not affected.
% % This feature was insofar exploited only at the application level, and transport protocols can significantly reduce the flow completion time by embracing such bounded loss-tolerance feature. 

\parab{Why a new transport-layer design?}
These desirable behaviors, however, do not match 
existing transport-layer techniques.
The mismatch stems from the {\em bounded loss 
tolerance} property exhibited by SGD-based training---the 
utility of a flow is determined by the time needed
to transfer a predefined fraction $p<100\%$ of all
data, not by the time to transfer all data.
In contrast, TCP and its variants seek to minimize the
time to transfer all data ($p=100\%$), which 
inevitably suffers from tail latency even under a 
tiny fraction of packet delays/losses.
UDP, on the other hand, does tolerate tail effect, 
but without the guarantee that at least $p$ data must
be delivered, which can result in poor eventual 
accuracy and/or require more iterations to converge.


% The bounded-loss tolerance of SGD has several significant implications for congestion control protocols. 
% First, it opens up new avenues to dramatically improving the congestion control performance.
% Traditionally, Reliable Data Transfer (RDT) protocols, e.g. TCP, are susceptible to even a tiny amount of packet losses or latency inflation, which can stall a flow with just a few retransmissions. 
% In contrast, SGD's inherent loss tolerance allows transport protocols to safely ignore packet losses or delays up to a certain amount ($10\%$ to $35\%$), which exceeds the packet loss rate seen in today's data centers. 
% This could dramatically cut the tail flow completion time.

% At the same time, we argue that imbuing the bounded loss tolerance in transport protocols calls for expanding the congestion control with a correspondingly new semantic.
% Instead of minimizing the flow completion time, a bounded-loss tolerant congestion control minimizes the time by which the receiver get a given fraction $p$ of all packets. 
% \footnote{Similar notion has been explored in early research on video streaming, sensor data aggregation, and redundant packet coding~\cite{rpt2012nsdi,sensor2002icdcs}, but as we will see, they are not directly applicable in high-speed data centers or for ML training. }
% This essentially points to a new utility function of a network flow---the utility of a network flow is determined by the time upon receiving a predefined fraction of data. 
% To our best knowledge, this is the first definition on bounded loss tolerance of transport protocol in data center settings.

In the rest of this short paper, we start with understanding the initial promise of a better transport-layer approach. Using large scale NS-3 simulations, we show a bounded-loss tolerance transport protocol can produce 1.1-2.2x speedup on different ML tasks under simplified assumptions. The simplified protocol significantly reduces the tail latency by tolerating bounded packet losses. 
With an analysis on the message contents of distributed ML jobs, we show a bounded-loss protocol can provide valid information for ML applications in presence of discrete packet drops. 
We then discuss related works and call upon this community to develop transport layer solutions for distributed ML leveraging such bounded-loss tolerance feature. 

% Stochastic Gradient Descent (SGD)-based optimization algorithms \cite{SGDopt,Adamopt,Momentumopt,Nesterovopt} are widely used in training models in machine learning~\cite{tensorflow,mxnet,petuum}. 
% but such SGD-based model training can be frustratingly slow, especially when many workers coordinate to train the same model.
% One reason is that large-scale distributed SGD requires intensive communication at the end of every iteration to synchronize and update huge amounts of parameters among the workers and a master server. 
